RLHF Can Speak Many Languages: Unlocking Multilingual Preference Optimization for LLMs

Preference optimization techniques have become a standard final stage for training state-of-art large language models (LLMs). However, despite widespread adoption, the vast majority of work to-date has focused on first-class citizen languages like English and Chinese. This captures a small fraction of the languages in the world, but also makes it unclear which aspects of current state-of-the-art research transfer to a multilingual setting. In this work, we perform an exhaustive study to achieve a new state-of-the-art in aligning multilingual LLMs. We introduce a novel, scalable method for generating high-quality multilingual feedback data to balance data coverage. We establish the benefits of cross-lingual transfer and increased dataset size in preference training. Our preference-trained model achieves a 54.4% win-rate against Aya 23 8B, the current state-of-the-art multilingual LLM in its parameter class, and a 69.5% win-rate or higher against widely used models like Gemma-1.1-7B-it, Llama-3-8B-Instruct, Mistral-7B-Instruct-v0.3. As a result of our study, we expand the frontier of alignment techniques to 23 languages covering half of the world's population.

==> sections/evaluation.tex <==
\section{Evaluation}
\ahmet{This should introduce how we evaluate the expeirments}

\textbf{Win rate evaluation}
Details of our evaluation datasets and settings

We evaluate preference optmized models on the Aya evaluation suite.


\textbf{Multilingual benchmarks}
Explain aya benchmark\citep{ustun2024aya,aryabumi2024aya}

==> tables/all_results.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llc|rrr|rrr|rrr}
\toprule
 &  & & \multicolumn{3}{c|}{\textbf{English}}  & \multicolumn{3}{c|}{\textbf{Avg. 5 Langs.}}   &  \multicolumn{3}{c}{\textbf{Avg. 23 Langs}}  \\
 & & \textbf{Num Examples} & 
\multicolumn{1}{c}{\textbf{Win\%}} & \multicolumn{1}{c}{\textbf{Loss\%}} & \multicolumn{1}{c|}{$\Delta$\textbf{W-L\%}} & 
\multicolumn{1}{c}{\textbf{Win\%}} & \multicolumn{1}{c}{\textbf{Loss\%}} & \multicolumn{1}{c|}{$\Delta$\textbf{W-L\%}} & 
\multicolumn{1}{c}{\textbf{Win\%}} & \multicolumn{1}{c}{\textbf{Loss\%}} & \multicolumn{1}{c}{$\Delta$\textbf{W-L\%}} \\ \midrule
& \textsc{EN-1} & 50K   & \multicolumn{1}{r}{52.0} & \multicolumn{1}{r}{33.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{92D3B3}18.5} & \multicolumn{1}{r}{43.8} & \multicolumn{1}{r}{38.7} & \multicolumn{1}{c|}{\cellcolor[HTML]{F4FBF8}5.1} & \multicolumn{1}{r}{43.7} & \multicolumn{1}{r}{40.1} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}3.6} \\
& \textsc{ML-5} & 50K & \multicolumn{1}{r}{50.5} & \multicolumn{1}{r}{28.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{79C9A1}22.0} & \multicolumn{1}{r}{45.3} & \multicolumn{1}{r}{37.7} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F4EB}7.6} & \multicolumn{1}{r}{43.9} & \multicolumn{1}{r}{39.1} & \multicolumn{1}{c}{\cellcolor[HTML]{F7FCF9}4.8} \\ 
& \textsc{ML-23} & 50K  & \multicolumn{1}{r}{44.5} & \multicolumn{1}{r}{36.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{DFF2E9}8.0} & \multicolumn{1}{r}{47.1} & \multicolumn{1}{r}{37.7} & \multicolumn{1}{c|}{\cellcolor[HTML]{D5EEE2}9.4} & \multicolumn{1}{r}{47.3} & \multicolumn{1}{r}{36.8} & \multicolumn{1}{c}{\cellcolor[HTML]{CDEBDC}10.5} \\ 
\multirow{-4}{*}{\textsc{DPO}} & \textsc{ML-23} & 230K & \multicolumn{1}{r}{57.5} & \multicolumn{1}{r}{31.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{57BB8A}26.5} & \multicolumn{1}{r}{52.1} & \multicolumn{1}{r}{37.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{AFDFC7}14.6} & \multicolumn{1}{r}{50.9} & \multicolumn{1}{r}{38.2} & \multicolumn{1}{c}{\cellcolor[HTML]{BDE4D1}12.7} \\  \midrule
& \textsc{EN-1} & 50K   & \multicolumn{1}{r}{47.5} & \multicolumn{1}{r}{38.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{D8EFE4}9.0} & \multicolumn{1}{r}{43.8} & \multicolumn{1}{r}{40.1} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}3.7} & \multicolumn{1}{r}{45.9} & \multicolumn{1}{r}{39.3} & \multicolumn{1}{c}{\cellcolor[HTML]{A0D9BD}6.6} \\
& \textsc{ML-5} & 50K & \multicolumn{1}{r}{55.5} & \multicolumn{1}{r}{30.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{63C092}25.0} & \multicolumn{1}{r}{52.5} & \multicolumn{1}{r}{37.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{A8DCC3}15.5} & \multicolumn{1}{r}{53.7} & \multicolumn{1}{r}{36.2} & \multicolumn{1}{c}{\cellcolor[HTML]{9AD6B8}17.5} \\ 
& \textsc{ML-23} & 50K & \multicolumn{1}{r}{53.0} & \multicolumn{1}{r}{37.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{A5DBC0}16.0} & \multicolumn{1}{r}{55.1} & \multicolumn{1}{r}{37.2} & \multicolumn{1}{c|}{\cellcolor[HTML]{97D5B6}17.9} & \multicolumn{1}{r}{54.0} & \multicolumn{1}{r}{38.0} & \multicolumn{1}{c}{\cellcolor[HTML]{A5DBC0}16.0} \\ 
\multirow{-4}{*}{\textsc{RLOO}} & \textsc{ML-23} & 230K^* & \multicolumn{1}{r}{53.0} & \multicolumn{1}{r}{35.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{96D5B6}18.0} & \multicolumn{1}{r}{54.9} & \multicolumn{1}{r}{35.1} & \multicolumn{1}{c|}{\cellcolor[HTML]{89CFAD}19.8} & \multicolumn{1}{r}{53.4} & \multicolumn{1}{r}{36.8} & \multicolumn{1}{c}{\cellcolor[HTML]{A0D9BD}16.6} \\
\bottomrule
\end{tabular}%
 }
\caption{We run multilingual preference optimization on multiple multilingual training dataset mixtures. Results are reported for DPO and RLOO preference optimization evaluated on open-ended generations from Aya evaluation suite \citep{ayadata2024}. Multilingual performance scales with the number of languages and the total number of examples in training data. We measure win-rates against the original Aya-23-8B \citep{aryabumi2024aya} using GPT-4-Turbo as a judge. We omit tie rates for brevity, as they can be calculated as Win\% + Loss\% + Tie\% = 100\%. EN-1, ML-5, ML-23 refer to English only, 5 languages (English, Vietnamese, Turkish, German, Portuguese), and 23 languages (Aya language list) respectively used in preference optimization.} 
\label{tab:dolly-overall-app}
\end{table*}

==> tables/comp_models.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|rrr|rrr|rrr}
\toprule
 & & \multicolumn{3}{c|}{\textbf{English}}  & \multicolumn{3}{c|}{\textbf{Avg. 5 Langs.}}   &  \multicolumn{3}{c}{\textbf{Avg. 23 Langs.}}  \\
 &  & 
\multicolumn{1}{c}{\textbf{Win\%}} & \multicolumn{1}{c}{\textbf{Loss\%}} & \multicolumn{1}{c|}{$\Delta$\textbf{W-L\%}} & 
\multicolumn{1}{c}{\textbf{Win\%}} & \multicolumn{1}{c}{\textbf{Loss\%}} & \multicolumn{1}{c|}{$\Delta$\textbf{W-L\%}} & 
\multicolumn{1}{c}{\textbf{Win\%}} & \multicolumn{1}{c}{\textbf{Loss\%}} & \multicolumn{1}{c}{$\Delta$\textbf{W-L\%}} \\ 
\midrule & 

\textsc{Gemma-1.1} & \multicolumn{1}{r}{36.5} & \multicolumn{1}{r}{57.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-20.5} &

\multicolumn{1}{r}{54.1} & \multicolumn{1}{r}{40.7} & \multicolumn{1}{c|}{13.4} &

\multicolumn{1}{r}{62.5} & \multicolumn{1}{r}{32.6} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}29.9} \\ 


& \textsc{Mistral-7B-v0.3} & \multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-} &

\multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{c|}{-} &

\multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}-} \\ 


\multirow{-3}{*}{\textsc{Base Aya 23}} & \textsc{Llama-3}  & \multicolumn{1}{r}{27.0} & \multicolumn{1}{r}{65.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-38.5} & 

\multicolumn{1}{r}{57.1} & \multicolumn{1}{r}{38.8} & \multicolumn{1}{c|}{18.3} & 

\multicolumn{1}{r}{67.4} & \multicolumn{1}{r}{28.2} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}39.2} \\


\midrule

& \textsc{Gemma-1.1}  & \multicolumn{1}{r}{46.5} & \multicolumn{1}{r}{45.5} & \multicolumn{1}{c|}{1.0} & 

\multicolumn{1}{r}{61.4} & \multicolumn{1}{r}{33.1} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}28.3} & 

\multicolumn{1}{r}{67.6} & \multicolumn{1}{r}{26.8} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}40.8} \\ 


& \textsc{Mistral-7B-v0.3} & \multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-} &

\multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{c|}{-} &

\multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}-} \\ 



\multirow{-2}{*}{\textsc{DPO}} & \textsc{Llama-3}  & \multicolumn{1}{r}{33.5} & \multicolumn{1}{r}{60.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-26.5} & \multicolumn{1}{r}{59.2} & \multicolumn{1}{r}{36.2} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}23.0} & \multicolumn{1}{r}{71.9} & \multicolumn{1}{r}{24.2} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}47.7} \\  


\midrule & 

\textsc{Gemma-1.1}  & \multicolumn{1}{r}{53.0} & \multicolumn{1}{r}{39.5} & \multicolumn{1}{c|}{13.5} & 

\multicolumn{1}{r}{64.7} & \multicolumn{1}{r}{30.6} & \multicolumn{1}{c|}{34.1} & 

\multicolumn{1}{r}{69.7} & \multicolumn{1}{r}{26.2} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}43.5} \\ 


& \textsc{Mistral-7B-v0.3} & \multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-} &

\multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{c|}{-} &

\multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}-} \\ 


\multirow{-2}{*}{\textsc{RLOO}} & \textsc{Llama-3} & \multicolumn{1}{r}{37.5} & \multicolumn{1}{r}{59.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-21.5} & 

\multicolumn{1}{r}{62.8} & \multicolumn{1}{r}{34.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}28.8} & 

\multicolumn{1}{r}{73.6} & \multicolumn{1}{r}{22.9} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}50.7} \\  


\bottomrule
\end{tabular}%
 }
\caption{Comparison against competitor models} 
\label{tab:gemma-overall}
\end{table*}

==> tables/en_main.tex <==
% \begin{table}[t]
% \centering
% \small
\setlength{\columnsep}{15pt}
\begin{wraptable}{R}{0.5\linewidth}
\centering
\vspace{-.5cm}
\fontsize{9.5}{9.5}\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{ll|rrr|}
\toprule
 &  & \multicolumn{3}{c}{\textbf{English}}    \\
 & &
\multicolumn{1}{c}{\textbf{Win\%}} & \multicolumn{1}{c}{\textbf{Loss\%}} & \multicolumn{1}{c}{$\Delta$\textbf{W-L\%}} \\ 

\midrule

& \textsc{EN-1}    & 
\multicolumn{1}{r}{52.0} & \multicolumn{1}{r}{33.5} & \multicolumn{1}{c}{\cellcolor[HTML]{A0D9BD}18.5} \\

& \textsc{ML-5}  & 
\multicolumn{1}{r}{50.5} & \multicolumn{1}{r}{28.5} & \multicolumn{1}{c}{\cellcolor[HTML]{80CCA7}22.0} \\ 

& \textsc{ML-23}   & 
\multicolumn{1}{r}{44.5} & \multicolumn{1}{r}{36.5} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}8.0} \\ 

\multirow{-4}{*}{\textsc{DPO}} & \textsc{ML-23*} & 
\multicolumn{1}{r}{57.5} & \multicolumn{1}{r}{31.0} & \multicolumn{1}{c}{\cellcolor[HTML]{57BB8A}26.5} \\  

\midrule

& \textsc{EN-1}    & 
\multicolumn{1}{r}{47.5} & \multicolumn{1}{r}{38.5} & \multicolumn{1}{c}{\cellcolor[HTML]{F6FCF9}9.0} \\

& \textsc{ML-5}  & 
\multicolumn{1}{r}{55.5} & \multicolumn{1}{r}{30.5} & \multicolumn{1}{c}{\cellcolor[HTML]{65C194}25.0} \\ 

& \textsc{ML-23}  & 
\multicolumn{1}{r}{53.0} & \multicolumn{1}{r}{37.0} & \multicolumn{1}{c}{\cellcolor[HTML]{B7E2CD}16.0} \\ 

\multirow{-4}{*}{\textsc{RLOO}} & \textsc{ML-23*}  & 
\multicolumn{1}{r}{53.0} & \multicolumn{1}{r}{35.0} & \multicolumn{1}{c}{\cellcolor[HTML]{A5DBC0}18.0} \\

\bottomrule
\end{tabular}

\caption{English Dolly win-rate results for DPO/RLOO preference optimized Aya 23 8B on multiple training data mixtures: EN-1 (English Only), ML-5 (5 Languages), ML-23 (23 Langauges). All runs are done with 50K total training examples with the exception of ML-23*, which is done with 230K total training examples. We report results for the best  checkpoint across 2 epochs.} 
\label{tab:en-main}
% \end{table}
\end{wraptable}

==> tables/ml_main.tex <==
% \begin{table}[t]
% \centering
% \small

\setlength{\columnsep}{15pt}
\begin{wraptable}{R}{0.5\linewidth}
\centering
\vspace{-.5cm}
\fontsize{9.5}{9.5}\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{ll|rrr|}
\toprule
 &  & \multicolumn{3}{c}{\textbf{Average 23 Languages}}    \\
 & &
\multicolumn{1}{c}{\textbf{Win\%}} & \multicolumn{1}{c}{\textbf{Loss\%}} & \multicolumn{1}{c}{$\Delta$\textbf{W-L\%}} \\ 

\midrule

& \textsc{EN-1}    & 
\multicolumn{1}{r}{43.3} & \multicolumn{1}{r}{40.6} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}2.7} \\

& \textsc{ML-5}  & 
\multicolumn{1}{r}{43.8} & \multicolumn{1}{r}{39.1} & \multicolumn{1}{c}{\cellcolor[HTML]{EAF7F1}4.7} \\ 

& \textsc{ML-23}   & 
\multicolumn{1}{r}{47.0} & \multicolumn{1}{r}{37.1} & \multicolumn{1}{c}{\cellcolor[HTML]{B3E1CB}9.9} \\ 

\multirow{-4}{*}{\textsc{DPO}} & \textsc{ML-23*} & 
\multicolumn{1}{r}{50.2} & \multicolumn{1}{r}{39.0} & \multicolumn{1}{c}{\cellcolor[HTML]{A6DBC1}11.2} \\  

\midrule

& \textsc{EN-1}    & 
\multicolumn{1}{r}{46.4} & \multicolumn{1}{r}{38.9} & \multicolumn{1}{c}{\cellcolor[HTML]{CDEBDC}7.5} \\

& \textsc{ML-5}  & 
\multicolumn{1}{r}{54.4} & \multicolumn{1}{r}{35.8} & \multicolumn{1}{c}{\cellcolor[HTML]{57BB8A}18.6} \\ 

& \textsc{ML-23}  & 
\multicolumn{1}{r}{54.0} & \multicolumn{1}{r}{38.0} & \multicolumn{1}{c}{\cellcolor[HTML]{73C79E}16.0} \\ 

\multirow{-4}{*}{\textsc{RLOO}} & \textsc{ML-23*}  & 
\multicolumn{1}{r}{53.4} & \multicolumn{1}{r}{37.0} & \multicolumn{1}{c}{\cellcolor[HTML]{6FC59B}16.4} \\

\bottomrule
\end{tabular}

\caption{Open-ended generation (Dolly) win-rates for DPO/RLOO preference optimized Aya models against the original Aya 23 8B. We report average win-rates on 23 languages for multiple training data mixtures: EN-1 (English Only), ML-5 (5 Languages), and ML-23 (23 Languages). All the data mixtures consist of 50K total training examples with the exception of ML-23*, which includes 230K total training examples. We report results for the best checkpoint across 2 epochs.} 
\label{tab:dolly-overall}
% \end{table}
\end{wraptable}

==> tables/xlsum.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llc|rrr|rrr|rrr}
\toprule
 &  & & \multicolumn{3}{c|}{\textbf{English}}  & \multicolumn{3}{c|}{\textbf{Avg. 4 Langs.}}   &  \multicolumn{3}{c}{\textbf{Avg. 15 Langs.}}  \\
 & & \textbf{Num Examples} & 
\multicolumn{1}{c}{\textbf{Win\%}} & \multicolumn{1}{c}{\textbf{Loss\%}} & \multicolumn{1}{c|}{$\Delta$\textbf{W-L\%}} & 
\multicolumn{1}{c}{\textbf{Win\%}} & \multicolumn{1}{c}{\textbf{Loss\%}} & \multicolumn{1}{c|}{$\Delta$\textbf{W-L\%}} & 
\multicolumn{1}{c}{\textbf{Win\%}} & \multicolumn{1}{c}{\textbf{Loss\%}} & \multicolumn{1}{c}{$\Delta$\textbf{W-L\%}} \\ \midrule
& \textsc{EN-1} & 50K   & \multicolumn{1}{r}{56.5} & \multicolumn{1}{r}{42.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{CAEADA}14.5} & \multicolumn{1}{r}{54.6} & \multicolumn{1}{r}{39.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{C8E9D9}15.1} & \multicolumn{1}{r}{52.5} & \multicolumn{1}{r}{41.6} & \multicolumn{1}{c}{\cellcolor[HTML]{D7EFE3}10.9} \\
& \textsc{ML-5} & 50K & \multicolumn{1}{r}{47.5} & \multicolumn{1}{r}{48.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{E67C73}-1.0} & \multicolumn{1}{r}{51.0} & \multicolumn{1}{r}{42.9} & \multicolumn{1}{c|}{\cellcolor[HTML]{E2F3EB}8.1} & \multicolumn{1}{r}{50.5} & \multicolumn{1}{r}{43.4} & \multicolumn{1}{c}{\cellcolor[HTML]{E5F5ED}7.1} \\ 
& \textsc{ML-23} & 50K  & \multicolumn{1}{r}{47.5} & \multicolumn{1}{r}{47.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.0} & \multicolumn{1}{r}{52.0} & \multicolumn{1}{r}{40.8} & \multicolumn{1}{c|}{\cellcolor[HTML]{D6EFE3}11.2} & \multicolumn{1}{r}{53.0} & \multicolumn{1}{r}{40.9} & \multicolumn{1}{c}{\cellcolor[HTML]{D3EDE0}12.1} \\ 
\multirow{-4}{*}{\textsc{DPO}} & \textsc{ML-23} & 230K & \multicolumn{1}{r}{56.5} & \multicolumn{1}{r}{41.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{C8E9D9}15.0} & \multicolumn{1}{r}{56.3} & \multicolumn{1}{r}{37.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{BAE3CF}18.8} & \multicolumn{1}{r}{56.7} & \multicolumn{1}{r}{37.5} & \multicolumn{1}{c}{\cellcolor[HTML]{B8E3CE}19.2} \\  \midrule
& \textsc{EN-1} & 50K   & \multicolumn{1}{r}{54.5} & \multicolumn{1}{r}{43.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{D5EEE2}11.5} & \multicolumn{1}{r}{57.4} & \multicolumn{1}{r}{36.6} & \multicolumn{1}{c|}{\cellcolor[HTML]{B3E0CA}20.8} & \multicolumn{1}{r}{58.0} & \multicolumn{1}{r}{35.8} & \multicolumn{1}{c}{\cellcolor[HTML]{ADDEC6}22.2} \\
& \textsc{ML-5} & 50K & \multicolumn{1}{r}{59.5} & \multicolumn{1}{r}{39.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{B5E2CC}20.0} & \multicolumn{1}{r}{62.1} & \multicolumn{1}{r}{32.9} & \multicolumn{1}{c|}{\cellcolor[HTML]{93D4B4}29.2} & \multicolumn{1}{r}{65.1} & \multicolumn{1}{r}{30.2} & \multicolumn{1}{c}{\cellcolor[HTML]{7ECBA6}34.9} \\ 
& \textsc{ML-23} & 50K & \multicolumn{1}{r}{61.0} & \multicolumn{1}{r}{36.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{A3DABF}25.0} & \multicolumn{1}{r}{68.6} & \multicolumn{1}{r}{28.1} & \multicolumn{1}{c|}{\cellcolor[HTML]{6AC397}40.5} & \multicolumn{1}{r}{70.7} & \multicolumn{1}{r}{25.3} & \multicolumn{1}{c}{\cellcolor[HTML]{57BB8A}45.4} \\ 
\multirow{-4}{*}{\textsc{RLOO}} & \textsc{ML-23} & 230K^* & \multicolumn{1}{r}{56.0} & \multicolumn{1}{r}{42.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCEBDB}14.0} & \multicolumn{1}{r}{64.9} & \multicolumn{1}{r}{31.4} & \multicolumn{1}{c|}{\cellcolor[HTML]{84CDA9}33.5} & \multicolumn{1}{r}{68.9} & \multicolumn{1}{r}{26.7} & \multicolumn{1}{c}{\cellcolor[HTML]{63C093}42.2} \\
\bottomrule
\end{tabular}%
 }
\caption{We run multilingual preference optimization on multiple multilingual training dataset mixtures. Results are reported for DPO and RLOO preference optimization evaluated on summarization from XLSum \citep{hasan-etal-2021-xl}. Multilingual performance scales with the number of languages and the total number of examples in training data. We measure win-rates against the original Aya-23-8B \citep{aryabumi2024aya} using GPT-4-Turbo as a judge. We omit tie rates for brevity, as they can be calculated as Win\% + Loss\% + Tie\% = 100\%. EN-1, ML-5, ML-23 refer to English only, 5 languages (English, Vietnamese, Turkish, German, Portuguese), and 23 languages (Aya language list) respectively used in preference optimization. \john{update with new numbers}} 
\label{tab:xlsum-overall}
\end{table*}
